Reinforcement Learning for Security-Aware Computation Offloading in Satellite Networks

The rise of NewSpace provides a platform for small and medium businesses to commercially launch and operate satellites in space. In contrast to traditional satellites, NewSpace provides the opportunity for delivering computing platforms in space. However, computational resources within space are usually expensive and satellites may not be able to compute all computational tasks locally. Computation Offloading (CO), a popular practice in Edge/Fog computing, could prove effective in saving energy and time in this resource-limited space ecosystem. However, CO alters the threat and risk profile of the system. In this paper, we analyse security issues in space systems and propose a security-aware algorithm for CO. Our method is based on the reinforcement learning technique, Deep Deterministic Policy Gradient (DDPG). We show, using Monte-Carlo simulations, that our algorithm is effective under a variety of environment and network conditions and provide novel insights into the challenge of optimised location of computation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Sat_Comm_IoTJ. <==
\glossaryentry{\textit {offloader}?\glossentry{off}|setentrycounter[]{page}\glsnumberformat}{5}


==> fig/fig_local.tex <==
\begin{tikzpicture}[>=latex,scale=1]


%\draw[step=1cm,gray,very thin] (-0,-0.9) grid (5.9,2.9);

%\node[anchor=north east]  {{CPU Utilisation(\%)}} at (0,4);
\node[align= right, below](t) at (2,-0.6cm){Time (Seconds)};
\node[align= center](ut) at (1,2.7cm){Resource Utilisation(\%)};

\draw[thick,->] (0,0) -- (4.5,0);
\draw[thick,->] (0,0) -- (0,2.5);
%[align=left, up] {CPU Utilisation(\%)};

\fill[fill=gray] (1,0) rectangle (3,2);

%\foreach \x in {1,3}
%\draw (\x cm,1pt) -- (\x cm,-1pt) node[anchor=north,fill=white] {$t_\x$};
\draw (1 cm,1pt) -- (1 cm,-1pt) node[anchor=north,fill=white] {$t_1$};
\draw (3 cm,1pt) -- (3 cm,-1pt) node[anchor=north,fill=white] {$t_2$};

\draw[thick,<->] (1 cm,1cm) -- (3 cm,1cm) node[midway,anchor=north] {$\tau_m$};
%\foreach \y in {1,2}
\draw (1pt,1 cm) -- (-1pt,1 cm) node[anchor=east,fill=white ] {$50$};
\draw (1pt,2 cm) -- (-1pt,2 cm) node[anchor=east,fill=white ] {$100$};

\end{tikzpicture}


==> fig/fig_offload.tex <==
\begin{tikzpicture}[>=latex,scale=0.8]


%\draw[step=1cm,gray,very thin] (-0,-0.9) grid (5.9,2.9);

%\node[anchor=north east]  {{CPU Utilisation(\%)}} at (0,4);
\def\xoff{-1}
\def\yoff{0}
\node[align= center](ut) at (2+\xoff,3.2cm){\textbf{\Gls{off}}};
\node[align= right, below](t) at (2+\xoff,-0.6cm){Time (Seconds)};
\node[align= center](ut) at (1+\xoff,2.7cm){ Utilisation(\%)};


\draw[thick,->] (0+\xoff,0) -- (4.5+\xoff,0);
\draw[thick,->] (0+\xoff,0) -- (0+\xoff,2.5);
%[align=left, up] {CPU Utilisation(\%)};
\def\ta{1}
\def\tb{1.5}
\def\tc{2}
\def\td{3}
\def\te{3.5}
\def\tf{4}

\fill[fill=gray] (\ta+\xoff,0) rectangle (\tb+\xoff,2);
\fill[fill=lightgray] (\tb+\xoff,0) rectangle (\tc+\xoff,2);
\fill[fill=gray] (\tc+\xoff,0) rectangle (\td+\xoff,0.2);

\fill[fill=lightgray] (\td+\xoff,0) rectangle (\te+\xoff,2);
\fill[fill=gray] (\te+\xoff,0) rectangle (\tf+\xoff,2);
%\fill[fill=gray] (1.5+\xoff,0) rectangle (2.5+\xoff,0.2);
%\filldraw[fill=gray, draw=black] (1,0) rectangle (3,2);
%\foreach \x in {0,1,2,3,4}
%\draw (\x cm+\xoff cm,1pt) -- (\x cm+\xoff cm,-1pt) node[anchor=north,fill=white] {$\x$};
\draw (\ta+\xoff ,1pt) -- (\ta+\xoff,-1pt) node[anchor=north,fill=white] {$t_1$};
\draw (\tb+\xoff ,1pt) -- (\tb+\xoff,-1pt) node[anchor=north,fill=white] {$t_2$};
\draw (\tc+\xoff ,1pt) -- (\tc+\xoff,-1pt) node[anchor=north,fill=white] {$t_3$};
\draw (\td+\xoff ,1pt) -- (\td+\xoff,-1pt) node[anchor=north,fill=white] {$t_4$};
\draw (\te+\xoff ,1pt) -- (\te+\xoff,-1pt) node[anchor=north,fill=white] {$t_5$};
\draw (\tf+\xoff ,1pt) -- (\tf+\xoff,-1pt) node[anchor=north,fill=white] {$t_6$};
\draw[thick,<->] (\ta+\xoff ,1cm) -- (\tb+\xoff ,1cm) node[midway,anchor=north] {$\tau_p$};
\draw[thick,<->] (\tb+\xoff ,1cm) -- (\tc+\xoff ,1cm) node[midway,anchor=north] {$\tau_s$};
\draw[thick,<->] (\tc+\xoff ,1cm) -- (\td+\xoff ,1cm) node[midway,anchor=north] {$\tau_w$};
\draw[thick,<->] (\td+\xoff ,1cm) -- (\te+\xoff ,1cm) node[midway,anchor=north] {$\tau_r$};
\draw[thick,<->] (\te+\xoff ,1cm) -- (\tf+\xoff ,1cm) node[midway,anchor=north] {$\tau_u$};
%\foreach \y in {1,2}
\draw (1pt+\xoff cm,1 cm) -- (-1pt+\xoff cm,1 cm) node[anchor=east,fill=white ] {$50$};
\draw (1pt+\xoff cm,2 cm) -- (-1pt+\xoff cm,2 cm) node[anchor=east,fill=white ] {$100$};

\end{tikzpicture}

==> fig/fig_system.tex <==
\begin{tikzpicture}[scale=0.85]
	\tikzset{satellite/.style={circle,
			color = black!70,
			minimum size = 1.8cm,
			inner sep = 0.1cm}}
\tikzset{satellitearrow/.style={-latex,
		line width = 0.125cm}}
			
%	\draw [ultra thick](4,5) circle (0.3cm) node[] (cloud) {C};
%	\draw [thick] (1,3) circle (0.3cm) node[] (e1) {E1};
	\draw [thick, rotate around={20:(0,6)}](-0.75,5.84) rectangle (0.75,6.16);
	\draw [thick,fill=white](0,6) circle (0.3cm) node[] (e2) {S};

%	\draw [thick](7,3) circle (0.3cm) node[] (e3) {E3};
%	\node (satellitea)  at (7, 1) [satellite, fill=yellow!50]   {A-STAR};
%	\draw (1,0) circle (0.3cm) node[] (d1) {D1};
	\draw (-84pt,95pt) rectangle (-72pt,75pt) node[left,above] (d2) {\footnotesize{V1}};
%	\draw (4,0) circle (0.3cm) node[] (d3) {D3};
	\draw (2pt,90pt) rectangle(12pt,70pt) node[above] (d4) {\footnotesize{V2}};
%	\draw (7,0) circle (0.3cm) node[] (d5) {D5};
	
	%\draw [bend right,dashdotted, red,thick,{Latex[length=3mm]}-{Latex[length=3mm]}](cloud) to (e1);
	%\draw [thick,dashdotted,red,{Latex[length=3mm]}-{Latex[length=3mm]}](cloud) to (e2);
	%\draw [bend left,dashdotted,red,thick,{Latex[length=3mm]}-{Latex[length=3mm]}](cloud) to (e3);
	%\draw [thick,dashed,blue,{Latex[length=3mm]}-{Latex[length=3mm]}](e1) to (e2);
	%\draw [thick,dashed,blue,{Latex[length=3mm]}-{Latex[length=3mm]}](e3) to (e2);
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e1) to (d1);	
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e1) to (d2);
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e2) to (d2);
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e2) to (d3);
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e3) to (d4);
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e3) to (d5);
	%\draw [thick,dotted,{Latex[length=3mm]}-{Latex[length=3mm]}](e2) to (d4);
	%\draw [bend right, thick,solid,<->](d5) to (d4);
	%\draw [thick,bend left,solid,<->](d3) to (d4);
	%\draw [thick, bend right,solid,<->](d3) to (d2);
	%\draw [thick,bend left,solid,<->](d1) to (d2);
	%\draw [bend right, thick,solid,<->](d1) to (d3);
	%\draw [bend left, thick,solid,<->](d5) to (d3);
	\draw [fill=darkgray](0,3) arc (0:180:1);
	\draw (1,3) arc (0:180:2);
	\draw [dash dot](0.5,3) arc (0:180:1.5);
%	\draw (0.5,3.4) arc (0:-80:2);
%	\draw (0.5,3.4) arc (0:80:2);
%	\draw [thick,solid,<->](cloud) to (e1);
%	\draw [thick,solid,<->](cloud) to (e2);
%	\draw [thick,solid,<->](cloud) to (e3);
%	\draw [thick,solid,<->](e1) to (e2);
%	\draw [thick,solid,<->](e3) to (e2);
%	\draw [thick,solid,<->](e1) to (d1);	
%	\draw [thick,solid,<->](e1) to (d2);
	\draw [thick,solid,<->](e2) to (d2);
%	\draw [thick,solid,<->](e2) to (d3);
%	\draw [thick,solid,<->](e3) to (d4);
%	\draw [thick,solid,<->](e3) to (d5);
	\draw [thick,solid,<->](e2) to (d4);
%	\draw [bend right,thick,solid,<->](d5) to (d4);
%	\draw [thick,bend left,solid,<->](d3) to (d4);
%	\draw [thick, bend right,solid,<->](d3) to (d2);
%	\draw [thick,bend left,solid,<->](d1) to (d2);
%	\draw [bend right, thick,solid,<->](d1) to (d3);
%	\draw [bend left, thick,solid,<->](d5) to (d3);
	
%	\draw[bend left=90,dashed,-{Latex[length=3mm]} ](d1)to node[auto, near start]{MCC} (cloud) ;
%	\draw[bend right=60,dashed,-{Latex[length=3mm]} ](d5)to node[right, near end]{MEC} (e3) ;
	
	\end{tikzpicture}

==> macros.tex <==
\setlength\unitlength{1mm}
\newcommand{\expectl}[2]{{\mathop{{\mathbb E}}}_{#1}\left[#2\right]}
\newcommand{\expect}[1]{{\mathop{{\mathbb E}}}\left[#1\right]}
\newcommand{\htp}{^{\sf H}}
\newcommand{\tp}{^{\sf T}}
\newcommand{\invm}[1]{\LB #1\RB^{-1}}
\newcommand{\inv}{^{-1}}
%\newtheorem{definition}{Definition}%[section]
\newtheorem{lemma}{Lemma}%[section]
%\newtheorem{cor}{Corollary}[section]
%\newtheorem{prop}{Proposition}
\newtheorem{defn}{Definition}[section]
%\newtheorem{conj}{Conjecture}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{remark}{\indent \bf Remark}[section]
%\newtheorem{property}{Property}[section]
\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{algorithm}{Algorithm}
\def\LSB{\left[}        %Left square bracketontrT)
\def\RSB{\right]}       %Right square bracket
\def\LB{\left(}         %Left bracket
\def\RB{\right)}        %Right bracket
\def\th{^\text{th}}

\newcommand{\asto}{\overset{\rm a.s.}{\longrightarrow}}






% bb font symbols

\newfont{\bbb}{msbm10 scaled 500}
\newcommand{\CCC}{\mbox{\bbb C}}

\newfont{\bb}{msbm10 scaled 1100}
\newcommand{\CC}{\mbox{\bb C}}
\newcommand{\RR}{\mbox{\bb R}}
\newcommand{\II}{\mbox{\bb I}}
\newcommand{\ZZ}{\mbox{\bb Z}}
\newcommand{\FF}{\mbox{\bb F}}
\newcommand{\GG}{\mbox{\bb G}}
\newcommand{\EE}{\mbox{\bb E}}
\newcommand{\NN}{\mbox{\bb N}}

% Vectors

\newcommand{\av}{{\bf a}}
\newcommand{\bv}{{\bf b}}
\newcommand{\cv}{{\bf c}}
\newcommand{\dv}{{\bf d}}
\newcommand{\ev}{{\bf e}}
\newcommand{\fv}{{\bf f}}
\newcommand{\gv}{{\bf g}}
\newcommand{\hv}{{\bf h}}
\newcommand{\iv}{{\bf i}}
\newcommand{\jv}{{\bf j}}
\newcommand{\kv}{{\bf k}}
\newcommand{\lv}{{\bf l}}
\newcommand{\mv}{{\bf m}}
\newcommand{\nv}{{\bf n}}
\newcommand{\ov}{{\bf o}}
\newcommand{\pv}{{\bf p}}
\newcommand{\qv}{{\bf q}}
\newcommand{\rv}{{\bf r}}
\newcommand{\sv}{{\bf s}}
\newcommand{\tv}{{\bf t}}
\newcommand{\uv}{{\bf u}}
\newcommand{\wv}{{\bf w}}
\newcommand{\vv}{{\bf v}}
\newcommand{\xv}{{\bf x}}
\newcommand{\yv}{{\bf y}}
\newcommand{\zv}{{\bf z}}
\newcommand{\zerov}{{\bf 0}}
\newcommand{\onev}{{\bf 1}}

% Matrices

\newcommand{\Am}{{\bf A}}
\newcommand{\Bm}{{\bf B}}
\newcommand{\Cm}{{\bf C}}
\newcommand{\Dm}{{\bf D}}
\newcommand{\Em}{{\bf E}}
\newcommand{\Fm}{{\bf F}}
\newcommand{\Gm}{{\bf G}}
\newcommand{\Hm}{{\bf H}}
\newcommand{\Id}{{\bf I}}
\newcommand{\Jm}{{\bf J}}
\newcommand{\Km}{{\bf K}}
\newcommand{\Lm}{{\bf L}}
\newcommand{\Mm}{{\bf M}}
\newcommand{\Nm}{{\bf N}}
\newcommand{\Om}{{\bf O}}
\newcommand{\Pm}{{\bf P}}
\newcommand{\Qm}{{\bf Q}}
\newcommand{\Rm}{{\bf R}}
\newcommand{\Sm}{{\bf S}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Um}{{\bf U}}
\newcommand{\Wm}{{\bf W}}
\newcommand{\Vm}{{\bf V}}
\newcommand{\Xm}{{\bf X}}
\newcommand{\Ym}{{\bf Y}}
\newcommand{\Zm}{{\bf Z}}

% Calligraphic

\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}

% Bold greek letters

\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\rhov}{\hbox{\boldmath$\rho$}}
\newcommand{\Psiv}{{\bf \Psi}}
\newcommand{\Upsilonv}{{\bf \Upsilon}}
\newcommand{\varphiv}{{\bf \varphi}}



\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}
\newcommand{\Mum}{\hbox{\boldmath$\Mu$}}

% mixed symbols
\newcommand{\rank}{{\hbox{rank}}}
\newcommand{\card}{{\hbox{card}}}
\newcommand{\sinc}{{\hbox{sinc}}}
\newcommand{\diag}{{\hbox{diag}}}
\renewcommand{\det}{{\hbox{det}}}
\newcommand{\trace}{{\hbox{tr}}}
\DeclareMathOperator{\tr}{tr}
\newcommand{\sign}{{\hbox{sign}}}
\renewcommand{\arg}{{\hbox{arg}}}
\newcommand{\var}{{\hbox{var}}}
\newcommand{\coh}{{\hbox{coh}}}
\newcommand{\SINR}{{\sf SINR}}
\newcommand{\SNR}{{\sf SNR}}
\newcommand{\Ei}{{\rm E}_{\rm i}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\eqdef}{\stackrel{\Delta}{=}}
\newcommand{\defines}{{\,\,\stackrel{\scriptscriptstyle \bigtriangleup}{=}\,\,}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}

